Using Hypotheses as a Debugging Aid

As developers debug, developers formulate hypotheses about the cause of the defect and gather evidence to test these hypotheses. To better understand the role of hypotheses in debugging, we conducted two studies. In a preliminary study, we found that, even with the benefit of modern internet resources, incorrect hypotheses can cause developers to investigate irrelevant information and block progress. We then conducted a controlled experiment where 20 developers debugged and recorded their hypotheses. We found that developers have few hypotheses, two per defect. Having a correct hypothesis early strongly predicted later success. We also studied the impact of two debugging aids: fault locations and potential hypotheses. Offering fault locations did not help developers formulate more correct hypotheses or debug more successfully. In contrast, offering potential hypotheses made developers six times more likely to succeed. These results demonstrate the potential of future debugging tools that enable finding and sharing relevant hypotheses.

==> sections/draft.tex <==
% Modern software development is built around APIs. Developers use and create APIs more than ever. The node.js package manager (knowing as npm), for example, hosts more than one million distinct libraries that developers download and use for more than three billion times each month. The enormous amount of libraries available makes it possible for developers to avoid building everything from scratch. In fact, the official npm blog post reported that ``97\% of the code in a modern web application comes from npm''. This means that web developers only need to build, debug, and test the remaining 3\% of their application. Another interesting new fact about modern APIs is that they are rapidly evolving. With the widespread embrace of agile development practices, libraries authors ship major updates more frequently. Java, for instance, has long been following more of a slow cycle that takes a couple of years to release new APIs. However, Oracle has recently announced that java is going to have new and non-trivial updates to its APIs every six months starting with the general availability of Java 10.

%Studies of debugging and code comprehension have identified the existence of hypotheses (e.g.,\cite{Brooks1983, Letovsky1987, VonMayrhauser1996}), but many questions remain about their influence within the debugging process. 

%Modern software development is heavily depended on many and rapidly evolving APIs. Debugging APIs is challenging due to the limited observability of the program state exaction, forcing developers into a practice known as \textit{black-box debugging}. In black-box debugging, developers construct a mapping between the inputs and outputs of APIs to formulate hypotheses. For example, a developer may use a visualization library to draw a shape by chaining multiple APIs to construct specific properties of the shape. If the shape has undesirable properties (e.g.color is black instead of white) or the shape does not render at all, developers may start reasoning about what APIs inputs caused the shape to have the undesirable properties. It is unexposed from developers to go inside the API implementation details and debug each line of code to gather information and hypothesize bout what causes the shape to have these  undesirable properties.



%  search queries are influenced by either error messages or a general query about APIs documentations, resulting sometimes in information that is not related to the defect they were facing.

%to how modern software development is heavily depended on many and rapidly evolving APIs \cite{npm2018}.


% Searching by error messages sometimes results in many explanations that were not the correct cause. When the defect did not output any error message, developers search for documentation and examples that sometimes did not highlight the error they were facing. 
% We note that their hypotheses also impact developers' query search. If their hypothesis is wrong, wasting time looking at irrelevant information that may not eventually lead them to a fix.

%more challenging. Developers will often find themselves using and debugging APIs that they are not entirely familiar with. While most debugging tools are more focus on helping developers step through their programs and check program state, debugging APIs are more focus on reasoning about inputs and outputs to APIs, a practice known as \textit{black-box debugging}. For example, a developer may use a visualization library to draw a shape by chaining multiple APIs to construct specific properties of the shape. If the shape has undesirable properties (e.g.color is black instead of white) or the shape does not render at all, developers may start construct a map between the inputs to the APIs and the output shape properties to arrive at a hypothesis about what causes the defect. If developers hypothesize that what causes the shape to be black is due wrong order of APIs calls, they may then edit input parameters, add more APIs calls or remove some of them to test their hypotheses.

% But are not able to construct a correct hypothesis when debugging APIs, they often interrupt their debugging work and turn to the internet (e.g., Stack Overflow and documentation) or seek help from an experienced coworker to find possible hypotheses about what might cause the defect. From a research perspective, this represents a time when developers need help in debugging APIs. To better understand the challenges developers face during this time,  we conducted a preliminary study by observing 5 hours of programming videos that show three professional developers working in three open-source projects. We note that their hypotheses also impact developers' query search. If their hypothesis is wrong, wasting time looking at irrelevant information that may not eventually lead them to a fix.

% One observation from this study is that developers may benefit from debugging tools that help them to construct the correct mental model defected APIs calls. Researchers have worked on providing a list of possible defect locations as debugging aid to help developers debug more effectively. Although there is still uncertainty around its usefulness as a debugging aid, it is still unknown how effective provide a location of the defected API call on helping developers constructing the correct mental model of the problem and form the correct hypothesis. Another possible way to help developers is by offering a list of possible hypotheses to them based on their APIs usage and the output they are receiving. These hypotheses are very general, representing coming defect dealing with APIs. For instance, a hypothesis for getting wrong shape color is that another code is changing the color of the shape. Another possible general hypothesis is that code is changing the color of the shape before construing the style property object of the shape. These are general hypotheses in that they are not including implantation details and can be shared with any developers using these APIs.  
